Character-aware Transformers Learn an Irregular Morphological Pattern Yet None Generalize Like Humans

Whether neural networks can serve as cognitive models of morphological learning remains an open question. Recent work has shown that encoder-decoder models can acquire irregular patterns, but evidence that they generalize these patterns like humans is mixed. We investigate this using the Spanish \emph{L-shaped morphome}, where only the first-person singular indicative (e.g., \textit{pongo} `I put') shares its stem with all subjunctive forms (e.g., \textit{ponga, pongas}) despite lacking apparent phonological, semantic, or syntactic motivation. We compare five encoder-decoder transformers varying along two dimensions: sequential vs. position-invariant positional encoding, and atomic vs. decomposed tag representations. Positional encoding proves decisive: position-invariant models recover the correct L-shaped paradigm clustering even when L-shaped verbs are scarce in training, whereas sequential positional encoding models only partially capture the pattern. Yet none of the models productively generalize this pattern to novel forms. Position-invariant models generalize the L-shaped stem across subjunctive cells but fail to extend it to the first-person singular indicative, producing a mood-based generalization rather than the L-shaped morphomic pattern. Humans do the opposite, generalizing preferentially to the first-person singular indicative over subjunctive forms. None of the models reproduce the human pattern, highlighting the gap between statistical pattern reproduction and morphological abstraction.

==> fig/accuracy_boxplot.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}

\begin{axis}[
axis lines=left,
grid=none,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Conditions},
xmin=0.5, xmax=3.5,
xtick style={color=black},
xtick={1,2,3},
xticklabels={10L\_90NL,50L\_50NL,90L\_10NL},
y grid style={darkgray176},
ylabel={Estimated Accuracy (\%)},
ymin=0, ymax=100,
ytick style={color=black}
]
\addplot [black]
table {%
0.85 32.685
1.15 32.685
1.15 50.8975
0.85 50.8975
0.85 32.685
};
\addplot [black]
table {%
1 32.685
1 17.84
};
\addplot [black]
table {%
1 50.8975
1 57.55
};
\addplot [black]
table {%
0.925 17.84
1.075 17.84
};
\addplot [black]
table {%
0.925 57.55
1.075 57.55
};
\addplot [black]
table {%
1.85 60.23
2.15 60.23
2.15 66.7575
1.85 66.7575
1.85 60.23
};
\addplot [black]
table {%
2 60.23
2 58.09
};
\addplot [black]
table {%
2 66.7575
2 70.16
};
\addplot [black]
table {%
1.925 58.09
2.075 58.09
};
\addplot [black]
table {%
1.925 70.16
2.075 70.16
};
\addplot [black]
table {%
2.85 68.73
3.15 68.73
3.15 72.285
2.85 72.285
2.85 68.73
};
\addplot [black]
table {%
3 68.73
3 64
};
\addplot [black]
table {%
3 72.285
3 76.1
};
\addplot [black]
table {%
2.925 64
3.075 64
};
\addplot [black]
table {%
2.925 76.1
3.075 76.1
};
\addplot [darkorange25512714]
table {%
0.85 44.86
1.15 44.86
};
\addplot [darkorange25512714]
table {%
1.85 60.885
2.15 60.885
};
\addplot [darkorange25512714]
table {%
2.85 70.27
3.15 70.27
};
\end{axis}

\end{tikzpicture}


==> fig/accuracy_boxplot_raw.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}

\begin{axis}[
axis lines=left,
grid=none,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Conditions},
xmin=0.5, xmax=3.5,
xtick style={color=black},
xtick={1,2,3},
xticklabels={10L-90NL,50L-50NL,90L-10NL},
y grid style={darkgray176},
ylabel={Accuracy (\%)},
ymin=0, ymax=100,
ytick style={color=black}
]
\addplot [black]
table {%
0.85 32.685
1.15 32.685
1.15 50.8975
0.85 50.8975
0.85 32.685
};
\addplot [black]
table {%
1 32.685
1 17.84
};
\addplot [black]
table {%
1 50.8975
1 57.55
};
\addplot [black]
table {%
0.925 17.84
1.075 17.84
};
\addplot [black]
table {%
0.925 57.55
1.075 57.55
};
\addplot [black]
table {%
1.85 60.23
2.15 60.23
2.15 66.7575
1.85 66.7575
1.85 60.23
};
\addplot [black]
table {%
2 60.23
2 58.09
};
\addplot [black]
table {%
2 66.7575
2 70.16
};
\addplot [black]
table {%
1.925 58.09
2.075 58.09
};
\addplot [black]
table {%
1.925 70.16
2.075 70.16
};
\addplot [black]
table {%
2.85 68.73
3.15 68.73
3.15 72.285
2.85 72.285
2.85 68.73
};
\addplot [black]
table {%
3 68.73
3 64
};
\addplot [black]
table {%
3 72.285
3 76.1
};
\addplot [black]
table {%
2.925 64
3.075 64
};
\addplot [black]
table {%
2.925 76.1
3.075 76.1
};
\addplot [darkorange25512714]
table {%
0.85 44.86
1.15 44.86
};
\addplot [darkorange25512714]
table {%
1.85 60.885
2.15 60.885
};
\addplot [darkorange25512714]
table {%
2.85 70.27
3.15 70.27
};
\end{axis}

\end{tikzpicture}

